Instrumenting Transaction Trace Properties in Smart Contracts: Extending the EVM for Real-Time Security

In the realm of smart contract security, transaction malice detection has been able to leverage properties of transaction traces to identify hacks with high accuracy. However, these methods cannot be applied in real-time to revert malicious transactions. Instead, smart contracts are often instrumented with some safety properties to enhance their security. However, these instrumentable safety properties are limited and fail to block certain types of hacks such as those which exploit read-only re-entrancy. This limitation primarily stems from the Ethereum Virtual Machine's (EVM) inability to allow a smart contract to read transaction traces in real-time. Additionally, these instrumentable safety properties can be gas-intensive, rendering them impractical for on-the-fly validation. To address these challenges, we propose modifications to both the EVM and Ethereum clients, enabling smart contracts to validate these transaction trace properties in real-time without affecting traditional EVM execution. We also use past-time linear temporal logic (PLTL) to formalize transaction trace properties, showcasing that most existing detection metrics can be expressed using PLTL. We also discuss the potential implications of our proposed modifications, emphasizing their capacity to significantly enhance smart contract security.

==> sections/logic.tex <==
\section{Logic}\label{sec:logic}

We use Quantified Computation Tree Logic \cite{DBLP:conf/concur/DavidLM16}.

\begin{definition}[$QCTL^*$]
Let $AP$ be a set of atomic propositions, and let $q,p \in AP$. 
The syntax of $QCTL^*$ is defined as follows:
$$\phi_s, \psi_s ::= q ~|~\lnot \phi_s \lor \psi_s~|~E\phi_p~|~A\phi_p~|~\exists p. \phi_s$$
$$\phi_p,\psi_p ::= \phi_s~|~\lnot\phi_p~|~\phi_p\lor\psi_p~|~X\phi_p~|~\phi_p U \psi _p$$
That is, $\phi_s, \psi_s \in QCTL^*$ and $\phi_p,\psi_p \in QCTL^*$.
Formulas $\phi_s$ and $\phi_s$ are called \emph{state formulas}, while $\phi_p$ and $\psi_p$ are called \emph{path formulas}.
The size of a formula $\psi \in QCTL^*$ is denoted by $|\psi|$ and is the number of steps needed to build $\psi$.
\end{definition}

Note that $CTL^*$ can be obtained from $QCTL^*$ by disallowing the rule $\exists p.\psi_s$.

The logics $QCTL$ and $CTL$ are obtained by using path formulas built with the following grammar:

$$\phi_p,\psi_p ::= X\phi_p~|~\phi_p U \psi _p$$




==> sections/states.tex <==
\section{System States}\label{sec:states}

We contract edges between states of the same Ethereum block that have the same contract A state, and add a loop to any nodes that resulted because of a contraction.
\todo[inline]{Change this above; we don't contract the CTL tree. Introduce CTL tree. Consider it optional to skip over nodes in a tree that don't result in a state change for the contract itself.}

General safety properties should be defined across the entire graph, but safety properties we care to check efficiently in Zircuit should be over a single column.

\input{figures/ctl-states-example-concrete}

\todo[inline]{Figure \ref{fig:states-example} -- what happens if we include gas related variables in the block? The phrase ``A state are contracted if they share the same block state variables'' will result in fewer contractions. Consider rephrasing that. Do accounts need to be in the system state boxes?}

Figure \ref{fig:all-states} shows concrete states -- those with concrete values for each variable. 
Abstracting these states away according to some properties is more important. 

Example abstract states are in Figure \ref{fig:abstract-states}, which represents a withdrawal of a contract of ERC-20 tokens. 
Throughout this example, we assume that ERC-20 tokens cannot be donated to the contract \texttt{A} that can receive them via a \texttt{deposit} function and return them to users via a \texttt{withdraw} function.
Let $D_s$ be all the transaction $d$ which called \texttt{deposit} function prior to reaching a state $s$.
When the \texttt{deposit} function is called, a user's \texttt{accountBalance} value is updated with the value deposited in the transaction $d$, denoted $d(v)$.
\texttt{accountBalance} is implemented as a mapping where the key is the user's Ethereum address, which is a $256$ bit number.

\todo[inline]{In this example, don't deal with ``multiple edges'' but take this figure as a snippet of the state machine for the contract only.}

\begin{figure*}
    \centering
\begin{tikzpicture}[font=\small, auto]
    % Define nodes
    \node[draw, rectangle, align=left] (state1) {$\sum_{i=0}^{2^{256}-1}  \texttt{accountBalance[}i \texttt{]} = \sum{d\in D_s}  v(d)$\\
    $\sum_{d\in D_s} v(d) = \texttt{balanceOf(C)}$};
    
    \node[draw, align=left, rectangle, below= 2.5cm of state1] (state2) {$\big(\sum_{i=0}^{2^{256}-1}  \texttt{accountBalance[}i\texttt{]}\big)-  \texttt{accountBalance[msg.sender]} = \big(\sum{d\in D_s} v(d)\big) - v(w)$\\
    $\sum_{d\in D_s} v(d) = \texttt{balanceOf(C)}$};
    
    %\node[draw, align=left, rectangle, below= 0.5cm of state2] (states2) {state $s+2$};
    %\node[below= 0.1cm of states2] (statesvdots) {$\vdots$};
    %\node[draw, align=left, rectangle, below= 0.1cm of statesvdots] (statesp) {state $s+|P|$};

    % Draw arrows 
    \draw[-latex] (state1) -- (state2) node[pos=0.5, left, align=left] {
    A withdrawal transaction $w$ of\\
    value \texttt{accountBalance[msg.sender]}\\ is called.
    The accounting in\\ the contract is updated \emph{before}\\ the tokens are actually transferred out.};
    %\draw[-latex] (state2) -- (states2); 
    %\draw[-latex] (statesp) to[out=270, in=180] (state1); 

    %\draw[-latex] (state2) to[out=135, in=180] (state1); 
    \draw[-latex] (state2) to[out=45, in=315] (state1); 
    \node[align=left] (rightLabel) at (3.25,-1.5) {
    After the accounting is updated, \\
    the token is transferred out\\ 
    and the previous state is entered.
    } ;
\end{tikzpicture}
    \caption{Abstract states during the withdrawal of an ERC-20 using the Checks-Effects-Interactions pattern (see e.g., \cite{ma2019fundamentals}). There is a multi-edge between the states as there are necessarily other state updates elsewhere (e.g., in the ERC-20 contract), but there may be multiple options if the ERC-20 contract makes other calls and changes other state on the blockchain.}
    \label{fig:abstract-states}
\end{figure*}
